Automatic Platform Configuration and Software Integration for Software-Defined Vehicles

In the automotive industry, platform configuration and software integration are mostly manual tasks performed during the development phase, requiring consideration of various safety and non-safety requirements. This manual process often leads to prolonged development cycles and provides limited flexibility. This paper introduces a novel approach to automate platform configuration and software integration for software-defined vehicles (SDVs), shifting these activities from the development phase to runtime. Our approach features an integration manager that combines model-based methods and virtualization technologies to generate and execute deployment plans. By leveraging model-based systems engineering (MBSE), our method automatically generates platform configuration and software integration plans, which are then converted into deployment-ready formats using code generation techniques. Utilizing virtualization and container orchestration technologies, the proposed system enables dynamic and flexible resource allocation while ensuring compliance with safety requirements. Communication between the development and runtime platforms is facilitated via a REST API. A proof of concept was implemented on a simulated SDV platform with the Intel Whiskey Lake Board. This demonstration showcases the integration manager on an SDV with a central computer, highlighting the potential to shorten development cycles and adapt to diverse vehicle configurations.

==> challenges.tex <==
The automated platform configuration and software integration in SDVs face various challenges.

One major challenge involves mapping hardware and software components for safety applications. 
In this paper we focus on SDVs with central computers.
Safety applications need to be allocated with required resources and at the same fulfill safety requirement, e.g., the freedom of interference. 
The software integration on traditional vehicles rely on statically defined resource distribution. 
For the software-defined vehicle, a flexible resource allocation is expected while safety requirements cannot be violated. 
This study aims to find architecture solutions for enabling applications with different safety levels running on the same central platform. 
To address this, we utilized both hardware-level and OS-level virtualization technologies, enabling the isolation of software execution environment.

Online solving and optimization present further challenges. Differing from traditional engineering processes, where vehicles are statically configured before being sold, SDVs should be able to determine their system configuration dynamically at runtime. It requires an optimization engine embedded in the vehicle.
In our previous work~\cite{Pan2022}, we propose a formal method of system description and optimization method for resource allocation in SDVs.
In this work, we aim to utilize this approach for the online solving on SDVs.
To ensure agile solving times that do not interfere with existing system software, we defined an incremental solving mechanism. 
